Unifying and extending Precision Recall metrics for assessing generative models

With the recent success of generative models in image and text, the evaluation of generative models has gained a lot of attention. Whereas most generative models are compared in terms of scalar values such as Frechet Inception Distance (FID) or Inception Score (IS), in the last years (Sajjadi et al., 2018) proposed a definition of precision-recall curve to characterize the closeness of two distributions. Since then, various approaches to precision and recall have seen the light (Kynkaanniemi et al., 2019; Naeem et al., 2020; Park & Kim, 2023). They center their attention on the extreme values of precision and recall, but apart from this fact, their ties are elusive. In this paper, we unify most of these approaches under the same umbrella, relying on the work of (Simon et al., 2019). Doing so, we were able not only to recover entire curves, but also to expose the sources of the accounted pitfalls of the concerned metrics. We also provide consistency results that go well beyond the ones presented in the corresponding literature. Last, we study the different behaviors of the curves obtained experimentally.

==> content/3_extensions_old.tex <==

\section{Analysis and unification of standard methods}

As seen in section \ref{section:precision-and-recall}, many different precision and recall methods for evaluating generative models have emerged and are defined within different contexts: while some output two scalar values as precision and recall, others represent precision and recall as trade-off curves, thus giving more refined information about the underlying distributions under comparison.
The key idea is using the dual approach to precision and recall, from \cite{simon_RevisitingPrecisionRecall_2019}, which expresses the PRD curve as an optimization problem on a family of binary classifiers (see equation \ref{eq:PR-Simon}).

We will now unfold our unifying framework where we extend the common scalar PR metrics to PR curves and discuss how this gives more information.



Let us first set the conventions with which we will be working. 

\subsection{Conventions used from then on}

The hypothesis we want to test is the following: $\mathcal{H}_0 = {z \sim P}$ (the null hypothesis).
The classifiers used are meant to distinguish the class from which the elements are taken:

\begin{itemize}
    \item for a classifier $f\in \mathscr{F}, f(z)=1 \iff z \sim P \iff \mathcal{H}_0 \equiv \textit{"negative sample"}$ 
    \item Conversely $f\in \mathscr{F}, f(z)=0 \iff z \sim Q \iff \Bar{\mathcal{H}_0} \equiv \textit{"positive sample"}$ 
\end{itemize}

\vspace{5mm}

This being set, we can define \textbf{misclassification} as follows:
\begin{itemize}
    \item False Positive (type I error) concerning classifier $f$: $z \sim P, f(z)=0$
    \item False Negative (type II error) concerning classifier $f$: $z \sim Q, f(z)=1$
\end{itemize}

\vspace{5mm}

Finally, the dual approach requires the use of \textbf{error rates}. Those are defined as follows:
\begin{itemize}
    \item False Positive Rate (fpr): $\fpr(f)=\frac{\|\{x \in \mathcal{X}, f(x)=0\}\|}{\|\mathcal{X}\|}$ (the fraction of elements from $\mathcal{X}$ -true samples- that are classified as being from $\mathcal{Y})$
    \item False Negative Rate (fnr): $\fnr(f)=\frac{\|\{y \in \mathcal{Y}, f(y)=1\}\|}{\|\mathcal{Y}\|}$ (the fraction of elements from $\mathcal{Y}$ -fake samples- that are classified as being from $\mathcal{X})$
\end{itemize}


\subsection{Analysis of commonly used precision and recall metrics and parallel with the dual version (\cite{simon_RevisitingPrecisionRecall_2019})}
\label{sec:analysis-of-pr-metrics}
Now our conventions are settled, we may build a parallel between the simple precision-recall metrics reviewed in \ref{section:common-precision-and-recall-metrics} and the extension proposed in \cite{simon_RevisitingPrecisionRecall_2019}.

In the alternative examples of precision and recall described before (\cite{kynkaanniemi_ImprovedPrecisionRecall_2019,naeem_ReliableFidelityDiversity_2020,park_ProbabilisticPrecisionRecall_2023}), the authors implicitly define a family of classifiers $\{f_0,f_\infty\}$ which are effectively used to compute a fpr and a fnr directly as precision and recall metrics.\\

\begin{itemize}
    \item For the computation of \textbf{precision}, the classifier is applied to all the generated samples and predicts if the generated samples fall within the support of the real distribution. This way, the classifier used is $f_\infty(z)=\1_{z \in \Bar{\mathcal{X}}}$ and the precision computed by the methods is the number of false negatives of that classifier $f$ i.e. the number of fake elements ($\sim \mathcal{Y}$) that are classified as real sample ($\sim \mathcal{X}$).
    \item In a symmetric fashion, the computation of \textbf{recall} is made by defining a new classifier $f_0(z)=\1_{z \in \Bar{Y}}$ that tries predicting if a sample comes from the estimation of distribution $\Bar{Y}$. Recall can be viewed as the fraction of elements from the real distribution that were predicted by the $f_0$ classifier as coming from the fake distribution. In other words, recall can be viewed as the false positive rate (fpr) of classifier $f_0$. 
\end{itemize}

Altogether, the described scalar precision-recall metrics are implicitly an expression of the dual approach (\ref{simon-dual-approach}), where the set of classifiers on which optimization is made is restrained to the two aforementioned classifiers $\F=\{f_0,f_\infty\}$. These methods employ a major bias in that for precision (resp. recall), the chosen classifier has a null fpr (resp. fnr): the classifier that predicts if $z \sim \P$ (resp. $z\sim \Q$) uses its own elements as a reference so it will not make a mistake. This bias is considerable as it means that the user is entirely convinced of the representativeness of the data distributions under study. We will later display our strategy to mitigate this issue by splitting the datasets into a training set on which the classifiers are built, and the test set on which the error rates are computed. With this method, there is \textit{a priori} no reason why the classifiers will have either null fpr or fnr. (This should also help the metrics to be more robust to outliers and to generalize better).

We can now construct the parallel between the 2 scalar-valued Precision and Recall and the PR curve based on the dual optimization problem from \cite{simon_RevisitingPrecisionRecall_2019}. Our goal therefore is -for a defined initial PR method- to build a custom lightweight family of classifiers $\mathcal{F}$ on which optimization can be made to yield the PRD points. Our main constraint is for the parametrized family of classifiers to output the two "extreme" classifiers for $\lambda = 0$ and $\lambda = +\infty$. To do so, we can thus create a parameterized family of classifiers, with a single scalar value $\gamma$ which will be equal at extreme values to the two classifiers discussed before.

\subsection{Extending "Improved Precision and Recall"}
As seen in section \ref{sec:analysis-of-pr-metrics}, the values of precision and recall defined in \cite{kynkaanniemi_ImprovedPrecisionRecall_2019} can be viewed as the max precision and max recall of a PRD curve, defined as the optimization within a class of binary classifiers. Also using \ref{algo:sajjadi-prd-algo}, it can be expressed in the following way:

\begin{align*}
    \alpha_{\max}&=\alpha_{\lambda \to \infty} = \sum_{\omega : Q(\omega) \neq 0 }P(\omega) \\
    \beta_{\max}&=\beta_{\lambda \to 0} = \sum_{\omega : P(\omega) \neq 0 }Q(\omega)
\end{align*}

Using the same notation as in the previous section, the extreme classifiers are the following:
\begin{align*}
    f_\infty &= z \mapsto \1_{z \in \bar{Y}} = \1_{\exists y \in \Y, z \in \BKNN^{\Y}(y)} \\
    f_0 &= z \mapsto \1_{z \in \bar{\X}} = \1_{\exists x \in \X, z \in \BKNN^{\X}(x)}
\end{align*}

We have thus constructed a family with only two classifiers. This still allows to explain what happens with the extreme points, yet we would like to interpolate the curve in order to extend it. To do so, we build the parameterized family of classifiers $\F_\ipr=\{f_\gamma^{\ipr}\}$ where:
\begin{equation}
    \label{eq:IPR-extension}
f_\gamma^{\ipr}= z \mapsto \1_{\tfrac{\gamma}{1+\gamma}\#\{x\in \X, z\in B_{kNN}^{\X}(x)\} \geq \tfrac{1}{1+\gamma}\#\{y\in \Y, z\in \BKNN^{\Y}(y)\} } 
\end{equation}

We have introduced the parameter $\gamma$ which still yields the same results for the two extreme points:
\begin{itemize}
    \item $f_{\gamma \to 0 } = z \mapsto \1_{\#\{x\in \X, z\in \BKNN^{\X}(x)\} \neq 0}  = $
\end{itemize}

\subsection{Link with Recall Cover}

\subsection{A probabilistic approach}


\section{Improving upon PRD curves extensions}

\subsection{True kNN classifier}
We saw in the previous section how to extend common precision-recall scalar metrics to PRD curves. Exploring the extension of \cite{naeem_ReliableFidelityDiversity_2020}, we also noticed how the estimation of the manifold was made using kNN balls, within $\X$ on the one hand and within $\Y$ on the other hand. Nevertheless, this is not the standard kNN classification. In order to properly export the kNN framework, we propose to compute kNN values within the family of classifiers on the union of the two sets $\X \cup \Y$. This way, we can decide the class to which a sample $z$ belongs based on a comparison of the number of elements of $\X$ that fall in $BKNN^{\X \cup \Y}(z)$ and the number of elements of $\Y$ that fall in that same ball.

\subsection{A call for splitting}
We described in Section \ref{sec:analysis-of-pr-metrics} how the metrics can be biased, based on the fact that the classifiers are defined and evaluated on the same datasets and any data point is included in its own knn ball. This is the reason why in the first order extension, for precision (resp. recall) the classifier has a null fpr (resp. fnr). While splitting datasets into train and test is a standard in the training of machine learning models, we reckon this should also be the case for the metrics that use such models and evaluate other generative models. In order to create the manifold estimations $\{\bar{\X},\bar{\Y}\}$, data points are used to define a collection of balls. We propose to first split the dataset into a train set which is used for the creation of the manifold estimation, and a test set on which the error rates are computed to yield the PRD curve. Splitting can be simply controlled by a train-test-ratio $r$ (we default that $r \in [0,1]$ means that no splitting occurs: the train and test samples are the same.\\

In the setting where a train and test split is used, the error rates are necessarily higher, which leads to an overestimation of the curve. 

\subsection{Visualization and comparison of the different manifold estimation methods}
\subsection{Experiments}

\section{}
